Semimartingales and Shrinkage of Filtration

We consider a complete probability space $(\Omega,\mathcal{F},\mathbb{P})$, which is endowed with two filtrations, $\mathbb{G}$ and $\mathbb{F}$, assumed to satisfy the usual conditions and such that $\mathbb{F} \subset \mathbb{G}$. On this probability space we consider a real valued special $\mathbb{G}$-semimartingale $X$. The purpose of this work is to study the following two problems: A. If $X$ is $\mathbb{F}$-adapted, compute the $\mathbb{F}$-semimartingale characteristics of $X$ in terms of the $\mathbb{G}$-semimartingale characteristics of $X$. B. If $X$ is not $\mathbb{F}$-adapted, given that the $\mathbb{F}$-optional projection of $X$ is a special semimartingale, compute the $\mathbb{F}$-semimartingale characteristics of $\mathbb{F}$-optional projection of $X$ in terms of the $\mathbb{G}$-canonical decomposition and $\mathbb{G}$-semimartingale characteristics of $X$.

==> preamble.tex <==
\usepackage{natbib}
\usepackage{rotating}
\usepackage{floatpag}
\rotfloatpagestyle{empty}

\usepackage{amsmath, amsfonts, amssymb, amsthm, bbm}
\usepackage{graphicx}
\usepackage{multind}\ProvidesPackage{multind}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{cancel}
\usepackage{color}
\usepackage{dsfont}
\usepackage[normalem]{ulem}
\usepackage[color=yellow, linecolor = red]{todonotes}
\usepackage{marginnote}

\usepackage[notref,notcite]{showkeys}
%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% nasze makra
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\app#1{\textcolor[rgb]{0.20,0.20,0.80}{#1}}
\def\mqed{\tag*{\qed}}
\def\I{\mathds{1}}
\newcommand{\set}[1]{{\left\{#1\right\}}}
\newcommand{\Set}[1]{\left\{#1\right\}} % set: {xyz} to be used for seapare (not inline) formulas
\newcommand{\abs}[1]{\left\|#1\right\|}
\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}

\usepackage{hyperref}
\def\mypart#1{}%{ \part{#1} }

\usepackage{t1enc}	

\usepackage{enumerate}
%\renewcommand*\labelenumi{\theenumi)}

\usepackage{graphicx}
% ----------------------------------------------------------------
\vfuzz2pt % Don't report over-full v-boxes if over-edge is small
\hfuzz2pt % Don't report over-full h-boxes if over-edge is small
% THEOREMS -------------------------------------------------------
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{varwidth}
%\usepackage{color}
%\usepackage[usenames]{color}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   Environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \newcommand\cambridge{EoM}
  \theoremstyle{plain}% default
  \newtheorem{theorem}{Theorem}[chapter]
  \newtheorem{lemma}[theorem]{Lemma}
  \newtheorem{proposition}[theorem]{Proposition}
  \newtheorem{corollary}[theorem]{Corollary}

  \theoremstyle{definition}
  \newtheorem{definition}[theorem]{Definition}
  \newtheorem{example}[theorem]{Example}
  \newtheorem{wyrostek}[theorem]{}
   \newtheorem{assumption}[theorem]{Assumption}


  \theoremstyle{remark}
  \newtheorem{remark}[theorem]{Remark}
  \newtheorem*{case}{Case}

  \setcounter{tocdepth}{2}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Stare environment'y
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bt}{\begin{theorem}}
\newcommand{\et}{\end{theorem}}
\newcommand{\bl}{\begin{lemma}}
\newcommand{\el}{\end{lemma}}
\newcommand{\bp}{\begin{proposition}}
\newcommand{\ep}{\end{proposition}}
\newcommand{\bd}{\begin{definition}}
\newcommand{\ed}{\end{definition}}
\newcommand{\bex}{\begin{example}}
\newcommand{\eex}{\end{example}}
\newcommand{\br}{\begin{remark}}
\newcommand{\er}{\end{remark}}
\newcommand{\brem}{\begin{remark}}
\newcommand{\erem}{\end{remark}}
\newcommand{\R}{\mathbb R}
\newcommand{\cJ}{\mathcal J}
\newcommand{\lab }{\label }
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bde}{\begin{displaymath}}
\newcommand{\ede}{\end{displaymath}}
\newcommand{\beq}{\begin{eqnarray*}}
\newcommand{\eeq}{\end{eqnarray*}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
\newcommand{\bea}{\begin{eqnarray*}}
\newcommand{\eea}{\end{eqnarray*}}
\newcommand{\1}{\mathbbm{1}}

%\newcommand{\mypart}[1]{}%\part{ #1 }}



\def\bal{\begin{aligned}}
\def\eal{\end{aligned}}
\def\bean{\equation\aligned}
\def\eean{\endaligned\endequation}
\def\bea{\equation\aligned\nonumber}
\def\eea{\endaligned\endequation}
%\def\be{\equation}
%\def\ee{\endequation}


\def \wh{\widehat}
\def \wt{\widetilde}
\def\r{\mathbb R}

\newcommand{\bplim}[1]{\mathop\textnormal{bp-lim}_{#1}}
\newcommand{\norm}[1]{\left\Vert#1\right\Vert}


% bigtimes
\DeclareFontFamily{U}{mathx}{\hyphenchar\font45}
\DeclareFontShape{U}{mathx}{m}{n}{
	<5> <6> <7> <8> <9> <10>
	<10.95> <12> <14.4> <17.28> <20.74> <24.88>
	mathx10
}{}
\DeclareSymbolFont{mathx}{U}{mathx}{m}{n}
\DeclareFontSubstitution{U}{mathx}{m}{n}
\DeclareMathSymbol{\bigtimes}{1}{mathx}{"91}
%end bigtimes
\DeclareMathAccent{\widebar}{0}{mathx}{"73}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%     Igor's macros
%% \mathcal Letters
\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}
\def\bcX{\mathbfcal{X}}
\def\bcbX{\bar{\mathbfcal{X}}}
\def\cMP{\mathcal{MP}}
\def\cMF{\mathcal{MF}}
\def\cMMP{\mathcal{MMP}}
\def\cMMF{\mathcal{MMF}}


%% \mathbb Letters
\def\bA{\mathbb{A}}
\def\bB{\mathbb{B}}
\def\bC{\mathbb{C}}
\def\bD{\mathbb{D}}
\def\bE{\mathbb{E}}
\def\bF{\mathbb{F}}
\def\bG{\mathbb{G}}
\def\bH{\mathbb{H}}
\def\bI{\mathbb{I}}
\def\bJ{\mathbb{J}}
\def\bK{\mathbb{K}}
\def\bL{\mathbb{L}}
\def\bM{\mathbb{M}}
\def\bN{\mathbb{N}}
\def\bO{\mathbb{O}}
\def\bP{\mathbb{P}}
\def\bQ{\mathbb{Q}}
\def\bR{\mathbb{R}}
\def\bS{\mathbb{S}}
\def\bT{\mathbb{T}}
\def\bU{\mathbb{U}}
\def\bV{\mathbb{V}}
\def\bW{\mathbb{W}}
\def\bX{\mathbb{X}}
\def\bY{\mathbb{Y}}
\def\bZ{\mathbb{Z}}

%% \mathbf Letters
\def\bfA{\mathbf{A}}
\def\bfB{\mathbf{B}}
\def\bfC{\mathbf{C}}
\def\bfD{\mathbf{D}}
\def\bfE{\mathbf{E}}
\def\bfF{\mathbf{F}}
\def\bfG{\mathbf{G}}
\def\bfH{\mathbf{H}}
\def\bfI{\mathbf{I}}
\def\bfJ{\mathbf{J}}
\def\bfK{\mathbf{K}}
\def\bfL{\mathbf{L}}
\def\bfM{\mathbf{M}}
\def\bfN{\mathbf{N}}
\def\bfO{\mathbf{O}}
\def\bfP{\mathbf{P}}
\def\bfQ{\mathbf{Q}}
\def\bfR{\mathbf{R}}
\def\bfS{\mathbf{S}}
\def\bfT{\mathbf{T}}
\def\bfU{\mathbf{U}}
\def\bfV{\mathbf{V}}
\def\bfW{\mathbf{W}}
\def\bfX{\mathbf{X}}
\def\bfY{\mathbf{Y}}
\def\bfZ{\mathbf{Z}}


\def\F{{\mathcal F}}
\def\H{{\mathcal H}}
\def\G{{\mathcal G}}
\def\X{{\mathcal X}}



\def\FF{{\mathbb F}}
\def\HH{{\mathbb H}}
\def\GG{{\mathbb G}}
\def\II{{\mathbb I}}
\def\XX{{\mathbb X}}


\def\P{\mathbb P}
\def\Q{\mathbb Q}
\def\QS{\mathbb Q^*}
\def\EP{{\mathbb E}_{\mathbb P}}
\def\EPS{{\mathbb E}_{\mathbb  P^*}}
\def\EQ{{\mathbb E}_{{\mathbb Q}}}
\def\EQS{{\mathbb E}_{\mathbb Q^*}}
\def\E {{\mathbb E} }
\def\tT{{t\in[0,T]}}
\def\uT{{u\in[0,T]}}


\def\wrt{\mbox{with respect to }}
\def\bla{\bea\bal}
\def\ela{\eal\eea}
%%%% fin macro %%%%
%\usepackage{todonotes}
\usepackage{marginnote}
\usepackage{fancyhdr}
\usepackage{lastpage}
  \pagestyle{fancy}
    \fancyhf{} % remove everything
    \renewcommand{\headrulewidth}{0pt} % remove lines as well
    \renewcommand{\footrulewidth}{0pt}
    \lhead{\texttt{\today}}
    %\chead{ Consistency and copulae theory for stochastic processes}
    \rhead{\thepage\ of \pageref{LastPage} }
%    \newcommand{\mn}[1]{\begin{color}{black}{#1}\end{color}}
 \def \cb { \textcolor {blue} }
 \def \cred { \textcolor {red} }

%%%%%%%%%%%%%%%%%%%%%%%% author predifined macros
\newcommand{\Mn}[1]{\begin{color}[rgb]{0.00, 0.0, 0.98}{\bf Mariusz:} #1 \end{color} }
\newcommand{\mn}[1]{\begin{color}[rgb]{0.00, 0.0, 0.98} #1 \end{color} }
\newcommand{\tr}[1]{\begin{color}[rgb]{1.00, 0.0, 0.00}{\bf Tomek:} #1 \end{color} }
\newcommand{\tm}[1]{\begin{color}[rgb]{1.00, 0.0, 0.00}{\bf Tomek and Mariusz:} #1 \end{color} }
\newcommand{\trb}[1]{\begin{color}[rgb]{0.50, 0.00, 0.50}{\bf TRB:} #1 \end{color} }


\newcommand{\jc}[1]{\begin{color}[rgb]{0.0, 0.50, 0.00}Jacek: #1 \end{color} }
\newcommand{\mj}[1]{\begin{color}[rgb]{0.00, 0.0, 0.98}Mariusz i Jacek : #1 \end{color}}
\newcommand{\jm}[1]{\begin{color}[rgb]{0.00, 0.0, 0.98}#1\end{color}}
%\newcommand{\jm}{}
%%%%%%%%%%%%%%%%%%%%%%%%
\def\bred{\bf \textcolor{red}  }
\def\mr{\textcolor{red}}
\def\mb{\textcolor{blue}}
\def\nieweglowski{Nieweg\l owski  }
\def\ja{\textcolor{green}}
%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\cadlag}{c\`{a}dl\`{a}g$\ $}


%%%%%%%%%%%%%%%%%%%%%%%%
 \mathchardef\mhyphen="2D


\definecolor{Bcolor}{rgb}{0,0.7,0}\def\Beh{\textcolor{Bcolor}}

